Quasi-projections in Teichm\"uller space

We consider a geometric property of the closest-points projection to a geodesic in Teichm\"uller space: the projection is called contracting if arbitrarily large balls away from the geodesic project to sets of bounded diameter. (This property always holds in negatively curved spaces.) It is shown here to hold if and only if the geodesic is precompact, i.e. its image in the moduli space is contained in a compact set. Some applications are given, e.g. to stability properties of certain quasi-geodesics in Teichm\"uller space, and to estimates of translation distance for pseudo-Anosov maps.

==> amsmacs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 			File name: amsmacs.tex
%% Macros for use with AMS-Latex. Contains theorem-environments 
%% and a proof environment with automatic labeling,
%% figure macros (including postscript), and assorted mathematical
%% abbreviations.   YNM 8/13/94
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Definitions that use @ : 
\catcode`\@=11

% Tiny marginpars 
\long\def\@savemarbox#1#2{\global\setbox#1\vtop{\hsize\marginparwidth 
%%%%%  \@parboxrestore #2}}
  \@parboxrestore\tiny\raggedright #2}}
\marginparwidth .75in \marginparsep 7pt 

\newcommand\lref[1]{\ref{#1}%
\@ifundefined{r@DisplaY #1}{}{(#1)}}% Prints label as well as
					 % number, if there is one.

\newcommand\fakelabel[2]{\@bsphack\if@filesw {\let\thepage\relax
   \newcommand\protect{\noexpand\noexpand\noexpand}%
\xdef\@gtempa{\write\@auxout{\string
      \newlabel{#1}{{#2}{\thepage}}}}}\@gtempa
   \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}

\catcode`\@=12

\def\Empty{}
\newcommand\oplabel[1]{
  \def\OpArg{#1} \ifx \OpArg\Empty {} \else
  	\label{#1}
  \fi}
% Here we define the numbering conventions for theorems, etc.
% They are all numbered together, consecutively in each section.
%
\newtheorem{theoremSt}{Theorem}[section]
\newtheorem{corollarySt}[theoremSt]{Corollary}
\newtheorem{propositionSt}[theoremSt]{Proposition}
\newtheorem{lemmaSt}[theoremSt]{Lemma}
\newtheorem{defineSt}[theoremSt]{Definition}
\newtheorem{exampleSt}[theoremSt]{Example}
\newtheorem{exerciseSt}[theoremSt]{Exercise}
\newtheorem{conjectureSt}[theoremSt]{Conjecture}
%
\newcommand\NextItem{\refstepcounter{theoremSt} \item[\thetheoremSt]}
% This macro allows us to define a bunch of similar theorem-environments
% with automatic labelling and extra features.
%
\newcommand\MakeStEnv[1]{
  \newenvironment{#1}[1]{%    environment without explicit label
  \begin{#1St} \oplabel{##1}%
  \global\def\CrntSt{\thetheoremSt}%
  %\def\Labl{##1}\ifx\Labl\Empty{} \else {\em (\Labl)\,}\fi%
  %%%{\em ##2}%
}{ 
  \end{#1St} }
  \newenvironment{#1+}[1]{%   environment with explicit label
  \begin{#1St} \label{##1}%
  \label{DisplaY ##1}%
  \global\def\CrntSt{\thetheoremSt}%
  \def\Labl{##1}\ifx\Labl\Empty{} \else {\em (\Labl)\,}\fi%
  %%%{\em ##2}%
}{ 
  \end{#1St} }
}
\MakeStEnv{theorem}
\MakeStEnv{corollary}
\MakeStEnv{proposition}
\MakeStEnv{lemma}
\MakeStEnv{define}
%%\MakeStEnv{example}  %% See below. 
\MakeStEnv{conjecture}

%% Define example environment without italics.
\newenvironment{example}[1]{%    environment without explicit label
  \begin{exampleSt} \oplabel{#1}%
  \global\def\CrntSt{\thetheoremSt}%
  \normalshape%
}{ 
  \end{exampleSt} }

\long\def\Restate#1#2#3{
\medskip\par\noindent
{\bf #1 \ref{#2}} {\rm(#2)}
{\it #3}
\par\medskip
}

\newcommand\restate[3]{
\medskip\par\noindent
{\bf #1 \ref{#2}} 
{\it #3}
\par\medskip
}

\long\def\retheorem#1#2{
\Restate{Theorem}{#1}{#2}}

\newenvironment{exercise}[1]{
  \small
  \begin{quote}	% To get indentation
    \begin{exerciseSt} \oplabel{#1}
    \rm
}{
    \end{exerciseSt}
  \end{quote}
  \medbreak\noindent
}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Insert a postscript figure using psfig.
% Usage:	\realfig{label}{filename}{caption}
%
% uses psfig macros: must have \input{psfig} in the preamble to use
% it. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\long\def\realfig#1#2#3{
\begin{figure}[htbp]
%%%\centerline{\psfig{figure=#3,height=#2}}
\centerline{\psfig{figure=#2}}
\caption[#1]{#3}
\oplabel{#1}
\end{figure}}
			 		
%
% Make a blank figure of given size with label in center.
% Usage:	\blankfig{label}{height}{caption}
%
\newlength{\saveu}
\newcommand\blankspace[2]{
  \setlength{\saveu}{#2}
  \divide\saveu by 2
  \vskip\saveu
%%  \centerline {\small \mbox{}#1}  %% label printing disabled
  \vskip\saveu
}

\long\def\placefig#1#2#3#4{
  \begin{figure}[#4]
    \blankspace{#1}{#2}
    \caption[#1]{#3}
    \oplabel{#1}
  \end{figure}}
\long\def\blankfig#1#2#3{
  \placefig{#1}{#2}{#3}{htbp}}
\long\def\herefig#1#2#3{
  \par\noindent\vbox{
  \blankspace{#1}{#2}
  \fakefigure\caption[#1]{#3}
  \oplabel{#1}
  \vspace{\intextsep}
  }}
\long\def\botfig#1#2#3{
  \placefig{#1}{#2}{#3}{b}}

%
\newenvironment{proof}[1]{%
  \def\PfArg{#1}
  \ifx\PfArg\Empty
  	\edef\PfArg{\CrntSt}  \fi
 {\parindent=0pt\startproof{\PfArg}}%
}{ 
  \finishproof{\PfArg}
}
%
\newcommand{\startproof}[1]{%
\medbreak\mbox{}\noindent{\it Proof of #1:}%
}
\newcommand{\finishproof}[1]{ 
  \def\FPArg{#1}
  \ifx\FPArg\Empty
  	\newcommand\FPArg{\CrntSt}  \fi
  \smallbreak\noindent\makebox[\textwidth]{\hfill\fbox{\FPArg}}
  \medbreak\noindent
}

\newcommand{\bfheading}[1]{\par\smallskip\noindent {\bf #1}}

%%% Assorted macros for mathematics formulas. 

\newcommand\tphi{|\til\Phi|}
\newcommand\phisig{{\aphi\over\sigma}}
\newcommand\phiavg{{\hbox{$\aphi$-Avg}}}
\newcommand\avg{\mathop{\hbox{Avg}}}
\newcommand\En{{\cal E}}
\newcommand\anu{{|\nu|}}
\newcommand\lnu{\log\anu}
\newcommand\Ssig{(S,\sigma)}
\newcommand\Srho{(S,\rho)}
\newcommand\PQ{{\bold PQ}}
\newcommand\rr{{\bold r}}
\newcommand\pp{{\bold p}}
\newcommand\AAA{{\cal A}}
\newcommand\BB{{\cal B}}
\newcommand\CC{{\cal C}}
\newcommand\DD{{\cal D}}
\newcommand\EE{{\cal E}}
\newcommand\FF{{\cal F}}
\newcommand\GG{{\cal G}}
\newcommand\HH{{\cal H}}
\newcommand\II{{\cal I}}
\newcommand\JJ{{\cal J}}
\newcommand\KK{{\cal K}}
\newcommand\LL{{\cal L}}
\newcommand\MM{{\cal M}}
\newcommand\NN{{\cal N}}
\newcommand\OO{{\cal O}}
\newcommand\PP{{\cal P}}
\newcommand\QQ{{\cal Q}}
\newcommand\RR{{\cal R}}
\newcommand\SS{{\cal S}}
\newcommand\TT{{\cal T}}
\newcommand\UU{{\cal U}}
\newcommand\VV{{\cal V}}
\newcommand\WW{{\cal W}}
\newcommand\XX{{\cal X}}
\newcommand\YY{{\cal Y}}
\newcommand\ZZ{{\cal Z}}
\newcommand\CH{{\CC\HH}}
\newcommand\MF{{\MM\FF}}
\newcommand\PMF{{\PP\MM\FF}}
\newcommand\ML{{\MM\LL}}
\newcommand\PML{{\PP\MM\LL}}
\newcommand\GL{{\GG\LL}}
\newcommand\Pol{{\cal P}}
\newcommand\half{{\textstyle{1\over2}}}
\newcommand\Half{{1\over2}}
\newcommand\Mod{\operatorname{Mod}}
\newcommand\Area{\operatorname{Area}}
\newcommand\dfd[1]{{\partial f\over \partial #1}}
\newcommand\zbar{{\overline{z}}}
\newcommand\wbar{{\overline{w}}}
\newcommand\phibar{{\overline{\Phi}}}
\newcommand\ep{\epsilon}
\newcommand\gep{{g_\epsilon}}
\newcommand\Mep{{M_\epsilon}}
\newcommand\iexp[1]{{\varepsilon(#1)}}
\newcommand\sexp{\varepsilon}
\newcommand\hhat{\widehat}
\newcommand\Proj{{\bold P}}
\newcommand\U{{\bold U}}
\newcommand\union{\cup}
\newcommand\intersect{\cap}
\newcommand\bbR{{\mathord{\text{I\kern-2pt R}}}}        % Fake blackboard
\newcommand\bbH{{\mathord{\text{I\kern-2pt H}}}}        % Fake blackboard

\newcommand\extendor{\raisebox{0ex}[0in][0in]{\rule{0.5pt}{4ex}}}

\newcommand\C{{\bold C}}
\newcommand\D{{\bold D}}
\newcommand\Z{{\bold Z}}
\newcommand\R{{\bold R}}
\newcommand\E{{\bold E}}
\newcommand\Hyp{{\bold H}}
\newcommand\Cstar{{\bold C_\ast}}
\newcommand\Rstar{{\bold R_\ast}}
\newcommand\RP[1]{{\bold RP}^{#1}}
\newcommand\PSL[1]{\text{PSL}_{#1}}
\newcommand\PSLtil[1]{\til\text{PSL}_{#1}}
\newcommand\PGL[1]{\text{PGL}_{#1}}
\newcommand\SL[1]{\text{SL}_{#1}}
%\newcommand\GL[1]{\text{GL}_{#1}}
\newcommand\CP[1]{{\bold CP}^{#1}}
\newcommand\SU[1]{\text{SU}(#1)}
\newcommand\PSU[1]{\text{PSU}(#1)}
\newcommand\SO[1]{\text{SO}(#1)}
%%%\newcommand\O[1]{\text{O}(#1)}
\newcommand\qi{{\bold i}}
\newcommand\qj{{\bold j}}
\newcommand\qk{{\bold k}}
\newcommand\diff{\hbox{\it Diff/}}

\newcommand\Longmapsto{\longmapsto}    % Eventually this should be improved 
\newcommand\bigrightarrow[1]{\hbox to #1{\rightarrowfill}}
\newcommand\bigleftarrow[1]{\hbox to #1{\leftarrowfill}}
%%\newcommand\iff{\Leftrightarrow}
\newcommand\Iff{\Longleftrightarrow}
\newcommand\homeo{\cong}
\newcommand\boundary{\partial}
\newcommand\semidir{\mathrel{\hbox{\vrule depth-.03ex height1.1ex\kern-0.15em$\times$}}}
\newcommand\isom{\hbox{isom}}
\newcommand\nbd{{\cal N}}
\newcommand\del{\nabla}
\newcommand\til{\widetilde}
\newcommand\length{\operatorname{length}}
\newcommand\tr{\text{tr}}
\newcommand\gesim{\succ}
\newcommand\lesim{\prec}
\newcommand\simle{\lesim}
\newcommand\simge{\gesim}
%%%\newcommand{\simmult}{\mathrel{\overset{\text{\tiny$\circ$}}{\sim}}}
\newcommand{\simmult}{\asymp}
\newcommand{\simadd}{\mathrel{\overset{\text{\tiny $+$}}{\sim}}}
\newcommand{\ssm}{\setminus}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\pair}[1]{\langle #1\rangle}

\numberwithin{equation}{section}


==> applications.tex <==
\section{Applications}
\label{applications}
We shall need the following immediate consequence of the contraction theorem: 
\begin{corollary}{easy corollary}
Let $L$ be an $\ep$-precompact geodesic in $\TT(S)$ and let $b_1,b_2$
be the constants given in theorem \ref{Contraction at a distance}. If
$R>b_1$ and points $x,y\in\TT(S)$ are connected by a path of length
$T$ which remains outside an $R$-neighborhood of $L$, then
\begin{equation}
\diam(\pi_L(x)\union \pi_L(y)) \le b_2\left({T\over R-b_1} + 1\right).
\label{path contraction}
\end{equation}
Furthermore for any $x,y\in\TT(S)$, 
\begin{equation}
\label{quasi lipschitz}
\diam(\pi_L(x)\union \pi_L(y)) \le d(x,y) + B(\ep).
\end{equation}
\end{corollary}
\begin{pf}
Dividing the path from $x$ to $y$ into pieces of size at most $R-b_1$
and applying theorem \ref{Contraction at a distance} yields 
inequality (\ref{path contraction}). To obtain (\ref{quasi
lipschitz}), let $R=2b_1$ and consider the 
geodesic $G$ connecting $x$ to $y$. If $G$ stays outside of an
$R$-neighborhood of $L$ then apply (\ref{path contraction}). If not, let
$x',y'$ be the closest points in $G$ to $x,y$ (respectively) such that
$d(x',L) = d(y',L) = R$. The triangle inequality together with
(\ref{path contraction}) yields
$$
\diam(\pi_L(x)\union\pi_L(y)) \le d(x,x') + 2R + d(x',y') + d(y,y') +
2b_2
$$
which suffices. 
\end{pf}

Define a {\em $(K,\delta)$-quasi-geodesic} in $\TT(S)$ as a path
$\Gamma:[a,b]\to\TT(S)$, 
parametrized by arclength, such that for any $s,t\in [a,b]$, 
$$|s-t|\le K d(\Gamma(s),\Gamma(t)) + \delta.$$ 

\begin{theorem}{Stability of quasi-geodesics}{}
Let $\Gamma$ be a $(K,\delta)$-quasi-geodesic path in $\TT(S)$, whose endpoints
are connected by an $\ep$-precompact Teichm\"uller geodesic $L$. Then
$\Gamma$ remains in a $B(K,\delta,\ep)$-neighborhood of $L$. 
\end{theorem}

\begin{pf}
The idea of the argument is standard:
any segment of $\Gamma$ which is
outside a sufficiently large neighborhood of $L$ is, because of 
the contractive properties of $\pi_L$, much less efficient than 
the path obtained by going back to $L$ and moving along the
projection. Thus large excursions from $L$ violate the quasi-geodesic property.

Fix $R = \max (Kb_2,2b_1)$.
Let $[s,t]$ be a maximal interval for which $\Gamma((s,t))$ is outside
an $R$-neighborhood 
of $L$.  Applying corollary \ref{easy corollary},
we have
$$ \diam(\pi_L(\gamma(s))\union\pi_L(\gamma(t)))\le {b_2\over 2R}|s-t|
+ b_2.$$
The maximality of $[s,t]$ implies that
$d(\Gamma(s),\pi_L(\Gamma(s))) = R$, and similarly for $t$. Thus
$$ d(\Gamma(s),\Gamma(t)) \le 2R + {b_2\over 2R}|s-t| + b_2$$
On the other hand, the
quasi-geodesic property of $\Gamma$ gives a lower bound on
the distance
$d(\Gamma(s),\Gamma(t))$, and together we obtain (using the definition
of $R$), a bound $|s-t| \le (4K+2)R + 2\delta$. 
It follows that $\Gamma$ cannot exit a $(2K+2)R+\delta$
neighborhood of $L$.
\end{pf}

\medskip

Let $\alpha$ be a measured foliation in $\MF(S)$.
The set 
$$Thin(\alpha,\delta) = \{\sigma\in\TT(S): E_\sigma(\alpha)\le\delta\}$$
is somewhat analogous to a horoball in hyperbolic space.
As in hyperbolic space, it has infinite diameter, but its projection
to a precompact geodesic is nevertheless bounded, bar one exceptional
case: 

\begin{theorem}{Cusp projections}{}
Given $\ep, \delta$ there is a constant $B$ such that, if $L$ is
a complete $\ep$-precompact geodesic and $\alpha\in\MF(S)$,
then
$$
\diam(\pi_L(Thin(\alpha,\delta)))\le B + \diam(L\intersect
Thin(\alpha,\delta)).
$$
\end{theorem}
Remarks: (1)
A special case of this is when $\alpha$ is a non-peripheral
simple closed  curve, with weight 1. Then $L\intersect Thin(\alpha,\delta)$
is uniformly bounded for all $\ep$-precompact $L$, so we have a
uniform bound on $\diam(\pi_L(Thin(\alpha,\delta)))$.
(2) If a complete geodesic $L$ is determined by a quadratic
differential $\Phi$, let us call $[\Phi_h]$ and $[\Phi_v]$ in
$\PMF(S)$ the {\em endpoints at infinity} for $L$. Another special
case occurs when $[\alpha]$ is equal in $\PMF(S)$ to an endpoint, and
then both sides of the inequality are infinite.


\begin{pf}{}
In view of remark (2), let us assume that $[\alpha] \ne
[\Phi_{h}],[\Phi_{v}]$ in $\PMF(S)$.
Masur proved in \cite{masur:uergodic} that, if $L$ is
$\ep$-precompact, then its 
endpoints at infinity are {\em uniquely ergodic} -- they support a
unique projective class of transverse measures. Thus the assumption
that $[\alpha]$ is not an endpoint implies that $\alpha$ is
topologically distinct from both foliations, and therefore (by lemma
\ref{Precompact implies complete}) it
intersects both of them non-trivially. It follows that $s_\alpha\ne
\pm\infty$ and that $E_t(\alpha)$ has a positive infimum, $E_0$.

Fix $\delta_0 < E_0c_1r_0$, where $c_1$ and $r_0$ are the constants
that appear in \S\ref{mM}.
We will show that $\pi_L(Thin(\alpha,\delta_0))$ lies in a
bounded neighborhood of $L(s_\alpha)$.

By the results of section \ref{mM}, it suffices to bound
$|s_\lambda-s_\alpha|$ for $\lambda\in\til A_{Mm}(\sigma,L)$, when
$\sigma\in Thin(\alpha,\delta_0)$. Suppose $|s_\lambda-s_\alpha|\ge
D$. Then by corollary \ref{product bound} we get
$$R_{s_\alpha}(\alpha)R_{s_\alpha}(\lambda) \le {1\over c_1}.$$
On the other hand, $R_{s_\alpha}(\alpha) \ge E_0/\delta_0$ by assumption, and
$R_{s_\alpha}(\lambda)\ge r_{s_\lambda}(\lambda)
\ge r_0$ as in lemma \ref{Ratio estimates distance},
so we obtain a contradiction. It follows that 
$|s_\lambda - s_\alpha|< D$.

\medskip

To prove the theorem for general $\delta > \delta_0$, we first observe that
$Thin(\alpha,\delta)$ lies in a neighborhood of
$Thin(\alpha,\delta_0)$ of radius $\half\log \delta/\delta_0$
(since one can move along a Teichm\"uller geodesic
defined by $\Phi$ such that $\Phi_h = \alpha$, and apply
(\ref{horizontal length})).

Applying corollary \ref{easy corollary} (inequality \ref{quasi
lipschitz}) we conclude immediately that the projection
$\pi_L(Thin(\alpha,\delta))$
lies in a $(C+\half\log\delta/\delta_0)$-neighborhood of
$L(s_\alpha)$, for an appropriate $C(\ep)$. On the other hand, 
applying lemma \ref{Extremal length estimate} and estimate (\ref{e is
exp}), we have $E_t(\alpha) \ge \half {E_0\over c_0} \exp 
2|t-s_\alpha|$. Using the definition of $E_0$, we have
$$
\diam (Thin(\alpha,\delta)\intersect L) \le \log {\delta\over\delta_0}
+ \log 2c_0c_1r_0.
$$
This completes the proof of the theorem. 
\end{pf}

Our last application is a geometric property of pseudo-Anosov
homeomorphisms. Let $f: S\to S$ be pseudo-Anosov, and let
$f_*$ denote the induced action on $\TT(S)$ (see
\cite{travaux} or \cite{abikoff}). Bers showed in  
\cite{bers:pseudoanosov} that the infimum $\inf_{\sigma\in
\TT(S)}d(\sigma,f_*\sigma)$
of translation distance is achieved in
$\TT(S)$ on a geodesic, namely the axis of $f_*$, on which
$f_*$ acts by translation.
The contraction theorem can be used to give lower bounds on how fast the
translation distance grows as we consider points far away from the
axis (this question was suggested by Feng Luo).

\begin{theorem}{pseudoanosov translation}
Let $f:S\to S$ be a pseudo-Anosov homeomorphism, and $L\subset \TT(S)$
the axis of $f_*$. There are $c_0,c_1>0$ such that, 
for all $x\in\TT(S)$,
$$
d(x,f_* x) \ge c_0 d(x,L) - c_1.
$$
\end{theorem}
Remark: it is easy to see that the rate of increase of $d(x,f_*x)$ is
at most linear with $d(x,L)$, and so in an asymptotic sense the
theorem gives maximal growth. However the constants $c_0$ and $c_1$
are completely non-constructive.

\begin{pf}
Since the axis $L$ is invariant by $f_*$, its image in the moduli
space is a closed curve, so that $L$ is precompact. 
Let $b_1,b_2$ be the constants given by theorem \ref{Contraction
at a distance} for $L$. 

For $x\in\TT(S)$, 
let $R = d(x,L)$ and let $t = d(x,f_*(x))$. Let $t_0$ denote the
translation distance of $f_*$ on $L$, so that $t\ge t_0$, and $t=t_0$
only for $x\in L$. 

For any $n>0$ we 
can connect $x$ to $f_*^nx$ by a chain of geodesics of length
$nt$, which remains outside an $R-t/2$ neighborhood of $L$. 
By corollary \ref{easy corollary} we have
$$
\diam(\pi_L(x)\union\pi_L(f_*^n x)) \le b_2\left({nt\over R-b_1-t/2} +
							1\right). 
$$
(Note that we may assume that $R-b_1-t/2 > 0$, because otherwise we
would have $t \ge 2R - b_1$, and we would be done.)
It follows that 
$$
d(x,f^n_*x) \le 2R + b_2\left({nt\over R-b_1-t/2} + 1\right).
$$
On the other hand $L$ is also the axis of $f^n_*$, so that 
$d(x,f^n_* x) \ge nt_0$. Letting $n$ go to infinity, we conclude that
$$
t_0 \le b_2{t\over R-b_1-t/2}.
$$
Solving for $t$, we obtain the desired inequality.
\end{pf}


==> front.tex <==
\title{Quasi-projections in Teichm\"uller space}
\author{Yair N. Minsky}
\address{Mathematics Department and IMS, SUNY Stony Brook, NY 11794}
\email{yair@math.sunysb.edu}
\date{November 23,1994}
%\thanks{}
%\subjclass{}

\maketitle





==> intro.tex <==
\newcommand{\Lbar}{\overline L}
\newcommand{\Str}{{\rm Stretch}}
\newcommand{\Mm}{\text{Maxmin}}
\newcommand{\mM}{\text{Minmax}}
\newcommand{\aaphi}{||\Phi||}
\newlabel{Slowmaps intersection lemma}{{3.2}{9}}

Many parallels have been drawn between geometric properties of the
Teichm\"uller space of a Riemann surface, and those of complete,
negatively curved spaces (see for example
Bers \cite{bers:pseudoanosov}, Kerckhoff \cite{kerckhoff:nielsen},
Masur \cite{masur:geoflow}, Wolpert \cite{wolpert:nielsen}). 
This paper investigates one such parallel --
the contracting properties of certain projections to geodesics.

We will use the Teichm\"uller metric throughout the paper (the other
famous metric on Teichm\"uller space, the Weil-Petersson metric, is
negatively curved although it is not complete -- see Wolpert
\cite{wolpert:noncomplete}. The Teichm\"uller 
metric is complete, but not negatively curved -- see Masur
\cite{masur:teichgeo}.) 

Every closed subset $C$ of a metric space $X$ determines
a ``closest-points'' projection,
defined as a map $\pi_C:X \to \PP(C)$, where $\PP(C)$ is the set
of closed subsets of $C$. Namely,
$$\pi_C(x) = \{y\in C:d(x,y) = d(x,C)\}$$
where $d(x,C) = \inf_{y\in C} d(x,y)$. (Provided $X$ is {\em proper},
i.e. $R$-balls are compact, $\pi_C(x)$ is never empty.)
Suppose now that $X$ is a
simply-connected Riemannian manifold with non-positive sectional
curvatures, and that $C$ is a geodesic segment, ray or line. In this
case $\pi_C(x)$ always consists of a single point. If the sectional
curvatures are bounded above by a negative constant, then 
$||d\pi_C||\to 0$ as $d(x,C)$ goes to $\infty$ (where $d\pi_C$ is the
differential of $\pi_C$). In other words, $\pi$ is
contracting at large distances. 

% A standard consequence of this is that ``quasi-geodesics'' are always
% in bounded neighborhoods of actual geodesics in such a space (see
% section \ref{applications}).
% 
\medskip

If $X=\TT(S)$, the Teichm\"uller space of a surface $S$ of finite
type, this contraction property fails in general, but a coarse form of
it can be shown to
hold for a special class of geodesics.
Call a geodesic (segment, ray, or line) $L$ in $\TT(S)$  {\em
precompact} if its 
projection to the moduli space $\MM(S)$ lies in a compact set. We say
$L$ is {\em $\ep$-precompact}  if $\ep>0$ is a lower bound on the
extremal length of any non-peripheral simple closed curve in $S$, for
any conformal structure in $L$ (see section \ref{preliminaries} for
definitions).  Our main theorem is the following: 

\restate{Theorem}{Contraction at a distance}{
Given $\ep$ there are constants $b_1,b_2$ depending on
$\ep,\chi(S)$ such that for any 
$\ep$-precompact geodesic $L$, if $\sigma\in \TT(S)$ is such that
$d(\sigma,L)> b_1$ then, setting $r=d(\sigma,L)-b_1$,
$$\diam(\pi_L(\nbd_r(\sigma)))\le b_2.$$
In particular, for some $b_0= b_0(\ep,\chi(S))$ and all
$\sigma\in\TT(S)$ we have
$$\diam(\pi_L(\sigma))\le b_0.$$
}

Here $\nbd_r$ denotes an $r$-neighborhood in the Teichm\"uller metric,
and we have taken the liberty of denoting by $\pi_L(A)$ the union
$\union_{a\in A}\pi_L(a)$.

Precompact geodesics are actually rare: by Masur's ergodicity
theorem \cite{masur:geoflow}, the infinite ones have zero measure in
the geodesic 
flow. In Theorem \ref{contraction converse} we show that Theorem
\ref{Contraction 
at a distance} is sharp, in the sense that it fails for all non-precompact
geodesics. 

Theorem \ref{Contraction at a distance} is a consequence of a
characterization of $\pi_L$ in 
terms of an extremal-length ratio problem. Minimizing the distance
of $\sigma\in\TT(S)$ to a geodesic $L$ is equivalent to solving the
problem of finding
$$\inf_{\tau\in L} \sup_\lambda {E_\tau(\lambda)\over
E_\sigma(\lambda)}$$
where the supremum is over $\lambda$ in $\PMF(S)$,
the set of projectivized measured
foliations of compact support in $S$. This is because the supremum of
extremal length ratios is just $\exp 2d(\sigma,\tau)$. In section
\ref{mM} we prove the following (stated a bit differently):

\restate{Theorem}{Characterize projection}{
If $\sigma\in\TT(S)$ and $L$ is $\ep$-precompact,
the points $\tau\in L$  which appear in the solutions of the dual problem
$$\sup_\lambda \inf_{\tau\in L} {E_\tau(\lambda)\over
E_\sigma(\lambda)}$$
are within a bounded distance of $\pi_L(\sigma)$. 
}


\medskip

In section \ref{applications} we give some consequences of
the contraction theorem, which are directly analogous to well-known properties
of hyperbolic space.
Theorem \ref{Stability of quasi-geodesics}
is a  ``stability'' property for a class of 
quasi-geodesics: a quasi-geodesic whose endpoints are connected by an
$\ep$-precompact geodesic must remain in a bounded neighborhood of the
geodesic. 
Theorem \ref{Cusp projections}
bounds the projected images of regions in Teichm\"uller
space which are analogous to horoballs in hyperbolic space. 
Theorem \ref{pseudoanosov translation}
is a lower bound for the translation distance of a pseudo-Anosov
automorphism of $\TT(S)$, in terms of distance from its axis; a
similar estimate holds for arbitrary loxodromic isometries in $\Hyp^n$.



==> mysty.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 			File name: mysty.tex
%% Macros for use in making my preprints with amslatex, but which 
%% shouldn't be included in electronic submission to a journal.
%% YNM 8/13/1994
%% Some changes in the heading macros 10/6/94
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Definitions that use @ : 
\catcode`\@=11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The following section definition is from AMSART.sty. It differs 
%% only in the indicated places, in order to allow sections to 
%% change the running heads, and to put a section symbol (\S) in front
%% of the section number (see defn of \@svsec)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@sect#1#2#3#4#5#6[#7]#8{%
\ifnum #2>\c@secnumdepth
   \let\@svsec\@empty
 \else
   \refstepcounter{#1}%
\edef\@svsec{\ifnum#2<\@m
             \@ifundefined{#1name}{}{\csname #1name\endcsname\ }\fi
%%%%% \noexpand\rom{\csname the#1\endcsname.}\enspace}\fi %%% (old line) 
\noexpand\rom{\S \csname the#1\endcsname.}\enspace}\fi
 \@tempskipa #5\relax
 \ifdim \@tempskipa>\z@ % then this is not a run-in section heading
   \begingroup #6\relax
   \@hangfrom{\hskip #3\relax\@svsec}{\interlinepenalty\@M #8\par}%
   \endgroup
%%%%%%% Old lines: %%%%%%%%%%%%%%%%%
%%%   \if@article\else\csname #1mark\endcsname{%
%%%     \ifnum \c@secnumdepth >#2\relax\csname the#1\endcsname. \fi#7}\fi
%%%%%%% Replacement lines: %%%%%%%%%
      \iffalse\else\csname #1mark\endcsname{%
     \ifnum \c@secnumdepth >#2\relax\@svsec\fi#7}\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifnum#2>\@m \else
       \addcontentsline{toc}{#1}%
{\ifnum #2>\c@secnumdepth \else
             \protect\numberline{%
               \ifnum#2<\@m
               \@ifundefined{#1name}{}{\csname #1name\endcsname\ }\fi
               \csname the#1\endcsname.}\fi
           #8}%
     \fi
 \else
  \def\@svsechd{#6\hskip #3\@svsec
    \@ifnotempty{#8}{\ignorespaces#8\unskip
       \ifnum\spacefactor<1001.\fi}%
        \ifnum#2>\@m \else
          \addcontentsline{toc}{#1}%
            {\ifnum #2>\c@secnumdepth \else
              \protect\numberline{%
                \ifnum#2<\@m
                \@ifundefined{#1name}{}{\csname #1name\endcsname\ }\fi
                \csname the#1\endcsname.}\fi
             #8}\fi}%
 \fi
\@xsect{#5}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Now the commands to produce the right running heads: 
%%
\def\@evenhead{\small\sc
      \rlap{\thepage}\hfil 
      \expandafter{\sh@rttitle}\hfil}%
% \def\@oddhead{\small\hfil
%     \expandafter\expandafter\expandafter\expandafter\expandafter
%     \expandafter\expandafter\uppercasetext@
%     \expandafter\expandafter\expandafter\expandafter\expandafter
%     \expandafter\expandafter{\rightmark}%
%     \hfil \llap{\thepage}}
 \def\@oddhead{\small \sc \mbox{}\hfil\hbox{\rightmark}\hfil 
       \llap{\thepage}}%
\let\sectionmark\markright

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section headings in bold instead of smallcaps.
%%
\def\section{\@startsection{\@string\section}%
        1\z@{9\p@\@plus12\p@}{6\p@}%
%%%     {\centering\defaultfont\sc}}
        {\centering\defaultfont\large\bf}}

\catcode`\@=12

%%% For the macintosh: redefined stuff
%%% \input{::tex:macintosh}

==> notation.tex <==
\section{Preliminaries}
\label{preliminaries}
We begin with a brief summary of results and notation. Let $S$ be a
surface of finite genus with finitely many punctures, and let $\TT(S)$
be the Teichm\"uller space of conformal structures of finite type on
$S$, where two structures are considered equivalent if there is a
conformal isomorphism of one to the other, which is isotopic to the
identity on $S$. By ``finite type'' we mean that each 
puncture has a neighborhood conformally equivalent to a punctured
disk. 

$\TT(S)$ has a natural topology, and is homeomorphic to a
finite-dimensional Euclidean space. The {\em Teichm\"uller distance}
between two points $\sigma,\tau\in\TT(S)$ is defined as 
$$d(\sigma,\tau) = \half\log K(\sigma,\tau),$$
where $K(\sigma,\tau)=K(\tau,\sigma)$ is the smallest possible quasi-conformal
dilatation of a homeomorphism from $(S,\sigma)$ to $(S,\tau)$ isotopic
to the identity. 

Let $\alpha$ be a homotopy class of simple closed curves in $S$.
Given $\sigma\in\TT(S)$, one may define the {\em extremal length} of
$\alpha$ in $\sigma$, as the inverse of the conformal modulus of the thickest
embedded annulus homotopic to $\alpha$ in $S$:
$$E_\sigma(\alpha) = \inf_{A\sim\alpha} {1\over{\rm Mod(A)}}.$$
This number is positive provided $\alpha$ is non-peripheral -- that
is, not deformable into a puncture. We will make heavy use of
Kerckhoff's theorem (see \cite{kerckhoff}), which states that 
\begin{equation}
K(\sigma,\tau) = \sup_\alpha {E_\tau(\alpha)\over E_\sigma(\alpha)}.
\label{K ratio}
\end{equation}

Kerckhoff in fact obtains this supremum as a maximum, by using a
completion of 
the space of homotopy classes of non-peripheral simple closed curves
known as the space of ``measured foliations with compact
support'', $\MF(S)$ (see \cite{travaux,levitt}). Elements of $\MF(S)$
are equivalence classes of foliations of $S$ with saddle singularities
(negative index) in the interior, and index 1/2 singularities at the
poles, equipped with transverse measures. The equivalence is via
isotopy, and saddle-collapsing (Whitehead) moves. $\MF(S)$ carries a
natural topology, and is homeomorphic to a Euclidean space of the same
dimension as $\TT(S)$. Multiplication of the measure by positive
scalars gives a ray structure to $\MF(S)$, and the quotient of
$\MF(S)$ (minus the empty foliation) by this multiplication is the
projectivized space $\PMF(S)$, which is a sphere. 

A homotopy class of simple closed curves, equipped with a real
number giving the 
measure, is represented in $\MF(S)$ as a foliation whose non-singular
leaves are in the homotopy class and fit together in a cylinder whose
height is the measure. These special foliations are dense in $\MF(S)$,
and Kerckhoff shows that
the extremal length function extends to a function
$E_\sigma(\lambda)$ which is continuous in both $\sigma$ and
$\lambda$, and scales quadratically:
$$E_\sigma(a\lambda) = a^2 E_\sigma(\lambda).$$
Moreover, the supremum in (\ref{K ratio}) is realized by a unique
projective class in $\PMF(S)$. 

Fixing $\sigma\in\TT(S)$, let $QD(S,\sigma)$ denote the space of
integrable holomorphic quadratic differentials on $(S,\sigma)$ (see
\cite{gardiner}). This
space may be identified with $\MF(S)$ by associating to a quadratic
differential $\Phi$ its horizontal foliation, which we call $\Phi_h$.
Hubbard-Masur \cite{hubbard-masur} showed that
this correspondence is a homeomorphism. From \cite{kerckhoff} we also 
have the equality
\begin{equation}
\label{length is mass}
E_\sigma(\Phi_h) = ||\Phi||
\end{equation}
where $||\Phi|| = \int_S|\Phi|$.
We note also that the vertical foliation $\Phi_v$, which is the
orthogonal foliation to $\Phi_h$, is just $(-\Phi)_h$. 

Geodesics in $\TT(S)$ are determined by holomorphic quadratic
differentials (and hence measured foliations) as
follows: Fix $\sigma\in\TT(S)$ and $\Phi\in QD(S,\sigma)$. The family
$\{\sigma_t\}_{t\ge 0}$
of conformal structures obtained by contracting along the leaves of
$\Phi_h$ by $e^t$ and expanding along $\Phi_v$ by $e^{-t}$, forms a
geodesic ray in the Teichm\"uller metric. Geodesics exist and are
unique between any two points in $\TT(S)$. We also have
$$d(\sigma,\sigma_t) = t$$
and
\begin{align}
\label{horizontal length}
E_{\sigma_t}(\Phi_h) &= e^{-2t} E_{\sigma}(\Phi_h), \\
\label{vertical length}
E_{\sigma_t}(\Phi_v) &= e^{2t} E_{\sigma}(\Phi_v).
\end{align}
\medskip

Our last group of definitions has to do with intersection number. The
standard  geometric (unoriented) intersection number between two simple closed
homotopy classes may be extended to a continuous function on
$\MF(S)\times\MF(S)$, homogenous in both arguments. One may best
visualize this in the case when one of the arguments is a simple
closed curve and the other is any measured foliation. The intersection
number is the smallest possible transverse measure deposited on a
homotopic representative of the simple closed curve.


Intersection numbers may be related to extremal lengths by the
following basic lemma which appears for example in
\cite{minsky:slowmaps}:
\begin{lemma}{Extremal length and intersection number}{}
If $\alpha, \beta$ are any two measured foliations on any Riemann
surface $X$, then
$$E_X(\alpha)E_X(\beta) \ge i(\alpha,\beta)^2.$$
\end{lemma}


We say a foliation $\lambda$ is {\em complete} if for any other
foliation $\mu$, $i(\lambda,\mu) = 0$ implies that the underlying leaf
structures of $\lambda$ and $\mu$ are the same (up to isotopy and
Whitehead moves). 

Let $L$ denote a geodesic segment, ray or line in $\TT(S)$. We say
that $L$ is {\em $\ep$-precompact}, for $\ep>0$, if for all $\tau\in L$ and
all non-peripheral simple closed curves $\gamma$ in $S$,
$E_\tau(\gamma)\ge\ep$. Equivalently, let $\MM(S)$ denote the moduli
space of $S$, which is the quotient of $\TT(S)$ by the induced action
of the group of homeomorphisms of $S$. A geodesic is precompact
exactly when its image in $\MM(S)$ is contained in a compact set. 

We will have need of another observation, which appears in
\cite{masur:teichgeo} and again in \cite{minsky:2d}:

\begin{lemma}{Precompact implies complete}
If $\Phi_h\in\MF(S)$ determines an $\ep$-precompact Teichm\"uller ray, then
$\Phi_h$ is complete. 
\end{lemma}






==> project.tex <==
\section{Two optimization problems}
\label{mM}
Let $L$ be an $\ep$-precompact geodesic segment, ray, or line and
let $\Lbar$ denote the complete geodesic line containing $L$. Choose an
arbitrary origin and orientation on $\Lbar$ and let the parameter $t$
denote signed distance from the origin. Then $L$ corresponds to an
interval $[a,b]$, where $-\infty\le a<b\le \infty$ (if $a=-\infty$ we
really mean $(-\infty,b]$, and similarly for $b=\infty$).
Denote by
$\Lbar(t)$ the conformal structure on $S$ given by the point
parametrized by $t$; or by $L(t)$ if $t\in[a,b]$.

\medskip

For each $\alpha\in\MF(S)$ and $t\in \R$, let $E_t(\alpha)$ be short for
the extremal length $E_{\Lbar(t)}(\alpha)$. 
Fixing a point
$\sigma\in\TT(S)$, define also 
$$R_{\sigma,t}(\alpha) = {E_t(\alpha)\over E_\sigma(\alpha)},$$
which we will tend to abbreviate as $R_t(\alpha)$.
Note that $R_t$ is invariant under scaling, making it a function
defined on projective classes in $\PMF(S)$. 

For each $t$ we have $d(\sigma,L(t)) = \half\log \sup_\alpha R_t(\alpha)$,
so finding $\pi_L(\sigma)$ reduces to minimizing this quantity over
$[a,b]$. 

Accordingly, define
\begin{eqnarray*}
\mM(\sigma,L) = \{(\alpha,t)\in\MF(S)\times[a,b]:
		R_t(\alpha) & = & \inf_s\sup_\beta R_s(\beta) \\
			 & = & \sup_\beta R_t(\beta)\}
\end{eqnarray*}
(where infima and suprema are over $[a,b]$ and $\MF(S)$,
respectively). Denote by $A_{mM}(\sigma,L)\subset \MF(S)$ the
projection of $\mM(\sigma,L)$ to its first factor, and let
$T_{mM}(\sigma,L)\subset[a,b]$ denote the projection of
$\mM(\sigma,L)$ to its second factor.
The projection $\pi_L(\sigma)$ is
exactly the set $\{L(t): t\in T_{mM}(\sigma,L)\}$.

Now consider the dual problem,
\begin{eqnarray*}
\Mm(\sigma,L) = \{(\alpha,t)\in\MF(S)\times[a,b]:
		R_t(\alpha) & = & \sup_\beta\inf_s R_s(\beta) \\
			 & = & \inf_s R_s(\alpha)\}
\end{eqnarray*}
and similarly define $T_{Mm}$ and $A_{Mm}$. 
Note that, in this problem, the first optimization, $\inf_s
R_s(\beta)$, is independent of $\sigma$. 
The main idea of this paper is to replace the Minmax problem with the
Maxmin problem. In particular,

\begin{theorem}{Characterize projection}{}
Let $L$ be an $\ep$-precompact geodesic in $\TT(S)$. Then for any
$\sigma\in \TT(S)$, 
$T_{mM}(\sigma,L)$ and $T_{Mm}(\sigma,L)$ have bounded
diameters, and are a bounded distance apart.
These bounds depend only  on $\ep$ and $\chi(S)$. 
\end{theorem}

\begin{pf}
The first step is to show that $E_t(\alpha)$, as a function of $t$, is
coarsely approximated by a strictly convex function. This in
particular will show that the minima of $E_t(\alpha)$ occur on
sets of bounded diameter. 

Let $\Phi$ be the holomorphic quadratic differential on $\Lbar(0)$
that determines the geodesic. The extremal lengths of the horizontal
and vertical foliations of $\Phi$ vary exponentially 
with $t$ according to (\ref{horizontal length}) and (\ref{vertical length}).
We also have $E_0(\Phi_h) = E_0(\Phi_v) = \aaphi$ by (\ref{length is
mass}), and we may normalize so that $\aaphi = 1$. 

We will need to know (see e.g. Gardiner-Masur \cite{gardiner-masur}) that
$\Phi_h$ and $\Phi_v$ {\em fill up $S$}, in the sense that every non-zero
element of 
$\MF(S)$ has positive intersection with at least one of them. 
Thus we may define the strictly positive function
$$e_t(\alpha) = \half\left({i(\alpha,\Phi_h)^2\over E_t(\Phi_h)}  + 
			   {i(\alpha,\Phi_v)^2\over E_t(\Phi_v)} \right)$$
which will serve as an approximation for $E_t(\alpha)$ (see lemma
\ref{Extremal length estimate}).

We can then introduce the following quantities, after fixing
$\sigma\in\TT(S)$. 
\begin{itemize}
\item
Let $s_\alpha$ denote the unique value of $t$ where
$e_t(\alpha)$ is minimal (possibly $s_\alpha = \infty$ or $-\infty$).
\item
Let $m(\alpha)$ be the set of $t$ values where $E_t(\alpha)$ is
minimal. 
\item Let $r_t(\alpha) = {e_t(\alpha)\over E_\sigma(\alpha)}.$
This function is an approximation for $R_t(\alpha)$, and takes its
minimum at $t=s_\alpha$. 
\item Let
${\til A_{Mm}}(\sigma,L) = \{[\alpha]\in\PMF(S): r_{s_\alpha}(\alpha) =
\max_{\beta\in\MF(S)} r_{s_\beta}(\beta)\}$.
\item Let
${\til T_{Mm}}(\sigma,L) = \{s_\alpha: [\alpha]\in{\til A_{Mm}}(\sigma,L)\}.$
\end{itemize}

Note that ${\til A_{Mm}}$ and ${\til T_{Mm}}$ are defined similarly to
$A_{Mm}$ and $T_{Mm}$, respectively, with $R_t$ replaced with $r_t$.
These definitions can be made for the following reason:
The function $r_t(\alpha)$
is invariant under scaling of $\alpha$, so it may be defined
for $[\alpha]\in\PMF(S)$. Since intersection number and extremal length
are continuous functions, it follows that the minimal values
$r_{s_\alpha}(\alpha)$ depend continously on $[\alpha]$. 
Therefore a  maximum is realized, since $\PMF(S)$ is compact.

The proof will divide into the following basic steps:
\begin{enumerate}
\item Show that $e_t(\alpha)$ and $r_t(\alpha)$ are approximations for
$E_t(\alpha)$ and $R_t(\alpha)$, respectively. As a consequence, the
set of minima $m(\alpha)$ is contained in a bounded neighborhood of
$s_\alpha$. 
\item Show that for a solution $\alpha\in A_{Mm}(\sigma,L)$ of the
Maxmin problem, $R_{s_\alpha}(\alpha)$ and $r_{s_\alpha}(\alpha)$ are
also good approximations to $\exp 2d(\sigma,L(s_\alpha))$. 
\item Conclude that $\diam \til T_{Mm}$ is bounded, and that $T_{Mm}$
and $T_{mM}$ lie in a bounded neighborhood of $\til T_{Mm}$. 
\end{enumerate}
Of these, step 2 contains the essential geometric idea of the paper,
and brings us most of the way to connecting the Maxmin and the Minmax
problems. 

Begin with this estimate:
\begin{lemma}{Extremal length estimate}{}
There is a fixed $c_0 = c_0(\ep,\chi(S))$ such that if $L$ is $\ep$-precompact
then for any $\alpha\in \MF(S)$ and $t\in[a,b]$,
$$e_t(\alpha)\le E_t(\alpha) \le c_0e_t(\alpha).$$
\end{lemma}

\begin{pf}{}
The left side actually does not depend on the precompactness of $L$ -- it
follows directly from lemma \ref{Extremal length and
intersection number}, applied to $\alpha$ and each of $\Phi_h$ and
$\Phi_v$. 

The right side follows from a compactness argument.  Let $\Phi^t$
denote the image of $\Phi$ in $L(t)$ under the Teichmuller map from
$L(0)$, scaled so that $||\Phi^t||=1$. Then as measured foliations we
have $\Phi^t_h = e^{-t}\Phi_h$ and $\Phi^t_v = e^{t}\Phi_v$. Thus,
$$e_t(\alpha) = \half\left(i(\alpha,\Phi^t_h)^2 +
i(\alpha,\Phi^t_v)^2\right).$$ 
The ratio $E_t(\alpha)/e_t(\alpha)$ is therefore a continuous positive function
of the projectivized measured foliation $[\alpha]\in\PMF(S)$ and the
pair $(L(t),\Phi^t)$ in the total space of Riemann surfaces equipped with
holomorphic quadratic differentials.
Fixing the Riemann surface $L(t)$, the space $\PMF(S)\times
PQD(L(t))$ is compact; and the function is invariant under the action
of the mapping class group. Further, the image of $L(t)$ in the
moduli space is restricted to a compact set by our definition of 
precompactness. It follows that $E_t(\alpha)/e_t(\alpha)$ is bounded.
\end{pf}{}

Now since $e_t(\alpha)$ is a strictly positive sum of
exponentials, a brief calculation using (\ref{horizontal
length},\ref{vertical length}) shows that,
excluding the case 
$s_\alpha=\pm \infty$, 
\begin{equation}
\half e_{s_\alpha}(\alpha) \exp 2|t-s_\alpha| \le e_t(\alpha) \le
2e_{s_\alpha}(\alpha) \exp 2|t-s_\alpha|
\label{e is exp}
\end{equation}
for $t\in[a,b]$.
It follows immediately from (\ref{e is exp}) and
lemma \ref{Extremal length estimate}
that $m(\alpha)$ is constrained by
\begin{equation}
m(\alpha) \subseteq [s_\alpha-\half\log2c_0,s_\alpha+\half\log2c_0].
\label{bound malpha}
\end{equation}
This concludes step 1 of the proof. 




Define
$$I_t(\alpha,\beta) = {i(\alpha,\beta)^2\over E_t(\alpha)E_t(\beta)}.$$

We begin the proof of step 2 with the following  crucial lemma. It
states that the minima 
$s_\alpha$ and $s_\beta$ for two measured foliations $\alpha,\beta$
can occur far apart only if $\alpha$ and $\beta$ are sufficiently
different to have a definite intersection number, as measured by
$I_t$:

\begin{lemma}{Distance implies intersection}{}
There are constants $D$ and $c_1$, depending only on $\ep$ and
$\chi(S)$, such that for any $\alpha,\beta\in\MF(S)$,
$$|s_\alpha - s_\beta| \ge D \quad\implies\quad 
I_{s_\alpha}(\alpha,\beta) \ge c_1.$$
\end{lemma}

\paragraph{Remark.}
This lemma is similar to (and was motivated by) lemma \ref{Slowmaps
intersection lemma} from \cite{minsky:slowmaps}, in which the role of $L$
is played by a hyperbolic 3-manifold $N$ homeomorphic to $S\times \R$,
and the role of the minimum point $s_\alpha$ is played by the geodesic
representative of $\alpha$ in $N$.

\begin{pf}{}
Suppose the lemma is false; then there exists a sequence of $\ep$-precompact
geodesics $L_i$ parametrized by $[a_i,b_i]$, with foliations
$\alpha_i$, $\beta_i$ such that $|s_{\alpha_i}-s_{\beta_i}|\to\infty$
while $I_{s_\alpha}(\alpha,\beta)\to 0$.

Adjusting if necessary by automorphisms of $S$, we may assume that the
points $L_i(s_{\alpha_i})$ lie in a fixed compact subset of a
fundamental domain of the action of the mapping class group on
$\TT(S)$. Further, the quantity $I_t$ is invariant under scaling of
the measures, and so is defined on the compact space
$\PMF(S)\times\PMF(S)$. Thus we may take a convergent subsequence and
obtain a limit example $(L,\alpha,\beta)$ in which
$I_{s_\alpha}(\alpha,\beta) = 0$, and $|s_\beta-s_\alpha|=\infty$.
Without loss of generality we assume $s_\beta = +\infty$, so that $L$
must contain an $\ep$-precompact ray $[s_\alpha,\infty)$. 

However, by lemma \ref{Precompact implies complete}, this implies that the
foliation $\Phi_h$ is complete. Since $s_\beta = +\infty$, we have
$i(\beta,\Phi_h) = 0$, so that $\beta$ must be topologically
equivalent to $\Phi_h$. On the other hand, the fact that $s_\alpha \ne
+\infty$ implies that $i(\alpha,\Phi_h)>0$, and therefore that
$i(\alpha,\beta)>0$, a contradiction.
\end{pf}

As a consequence of this lemma we can show that
two foliations with sufficiently distant minima cannot 
both give a large minimal value for $R_t$. 

\begin{corollary}{product bound}
For any $\alpha,\beta\in \MF(S)$, 
if $|s_\alpha - s_\beta| > D$ then 
$$
	R_{s_\alpha}(\alpha) R_{s_\alpha}(\beta) \le 1/c_1
$$
where $D,c_1$ are the constants of lemma \ref{Distance implies intersection}.
\end{corollary}

\begin{pf}
Lemma \ref{Distance implies intersection} implies that 
$
i(\alpha,\beta)^2 \ge c_1 E_{s_\alpha}(\alpha) E_{s_\alpha}(\beta).
$
On the other hand, lemma \ref{Extremal length and intersection number}
assures us that 
$
	E_\sigma(\alpha)E_\sigma(\beta)\ge i(\alpha,\beta)^2.
$
Combining these inequalities yields the desired conclusion.
\end{pf}

\medskip

We can now complete step 2 of the proof: 
\begin{lemma}{Ratio estimates distance}{}
There exists a constant $c_3(\ep,\chi(S))$ such that
$$
	R_{s_\lambda}(\lambda) \le \exp 2d(\sigma,L(s_\lambda)) \le
	c_3R_{s_\lambda}(\lambda)
$$ 
for $[\lambda]\in {\til A_{Mm}}(\sigma,L)$.
\end{lemma}

\begin{pf}{}
The left side of the inequality is immediate from (\ref{K ratio}).

Let
$[\mu]\in\PMF(S)$ denote the unique projective class of measured
foliations, such that  
$$d(\sigma,L(s_\lambda)) = \half\log R_{s_\lambda}(\mu),$$
and, in particular, $[\mu]$ maximizes $R_{s_\lambda}$ over $\PMF(S)$.
Thus our job is to find an upper bound for the ratio
$$Q = R_{s_\lambda}(\mu) / R_{s_\lambda}(\lambda).$$
The idea will be that, if $Q$ is large, then by the exponential growth
of $e_t$ and the fact that the minimum of $r_t(\mu)$ is no
larger than the minimum of $r_t(\lambda)$,
we may conclude that $|s_\lambda-s_\mu|$ is large. But then
corollary \ref{product bound} implies that $R_{s_\lambda}(\lambda)$
and $R_{s_\lambda}(\mu)$ cannot both be large, which will yield a
contradiction. 

By virtue of the estimate (\ref{e is exp}) on $e_t$, we have
$$r_{s_\lambda}(\mu) \le 2 e^{2|s_\lambda-s_\mu|}r_{s_\mu}(\mu).$$
Lemma \ref{Extremal length estimate} implies that
$R_{s_\lambda}(\mu) \le c_0r_{s_\lambda}(\mu)$, and by choice of
$\lambda$ we have $r_{s_\mu}(\mu)\le r_{s_\lambda}(\lambda)\le
R_{s_\lambda}(\lambda)$. Therefore we conclude
$$Q\le {2c_0} e^{2|s_\lambda-s_\mu|},$$
or
$$|s_\lambda-s_\mu| \ge \half\log Q/2c_0.$$
Now suppose $Q\ge 2c_0\exp 2D$, with $D$ the constant from lemma
\lref{Distance implies intersection}. Corollary \ref{product bound}
implies that 
$$
R_{s_\lambda}(\lambda)R_{s_\lambda}(\mu) \le {1\over c_1}
$$
and hence
$$
Q\le (c_1R^2_{s_\lambda}(\lambda))^{-1}.
$$
To bound $Q$ we need only note that there is a lower bound for
$R_{s_\lambda}(\lambda)$: There is a constant $\ell_0$ depending on
$\chi(S)$ such that the shortest simple closed curve $\alpha$ on $S$
has $E_\sigma(\alpha)\le \ell_0$. Since $L$ is $\ep$-precompact,
$R_t(\alpha)\ge \ep/\ell_0$ for all $t\in[a,b]$. 
Tracing through our definitions, 
it follows that $r_{s_\alpha}(\alpha) \ge r_0 = \ep/\ell_0c_0$, and hence
that 
$R_{s_\lambda}(\lambda)\ge  \ep/\ell_0c_0$ as well. This gives the desired
bound on $Q$.
\end{pf}

\medskip

We proceed with the proof of step 3, and bound
the diameter of
${\til T_{Mm}}(\sigma,L)$. Suppose
$\lambda,\mu\in{\til A_{Mm}}(\sigma,L)$. 
If $|s_\lambda-s_\mu|\ge D$
then corollary \ref{product bound} bounds
$R_{s_\lambda}(\lambda)R_{s_\lambda}(\mu)$. 

On the other hand,
$R_{s_\lambda}(\lambda) \ge r_{s_\lambda}(\lambda)$, and by (\ref{e is exp})
$R_{s_\lambda}(\mu) \ge \half r_{s_\mu}(\mu)\exp|s_\lambda-s_\mu|$.
Since, as in the previous proof,
$r_{s_\lambda}(\lambda)=r_{s_\mu}(\mu)\ge r_0$ for a fixed $r_0$,  we
get
$$\half r_0^2 e^{2|s_\lambda-s_\mu|} \le {1\over c_1}$$
which bounds $|s_\lambda-s_\mu|$ by some $c_4$. 

Similarly, if $\lambda\in{\til A_{Mm}}(\sigma,L)$ and $\mu\in A_{Mm}(\sigma,L)$
then $\inf_t R_t(\mu)$ is maximal in $\MF(S)$ and in particular is at
least $r_0$. Thus we may repeat the argument of the previous
paragraph to obtain a bound on $|s_\lambda-s_\mu|$ in this case as
well.

Using the bound (\ref{bound malpha}) on $m(\alpha)$ in terms of
$s_\alpha$, and the fact that
$T_{Mm}(\sigma,L) = \bigcup_{\alpha\in A_{Mm}(\sigma,L)} m(\alpha)$,
we conclude that $T_{Mm}(\sigma,L)$ lies in a
bounded neighborhood of ${\til T_{Mm}}(\sigma,L)$, and thus its diameter is
bounded, and half the theorem is proven.

\medskip

To complete the proof, we must show that 
$T_{mM}(\sigma,L)$ is in a bounded neighborhood of ${\til
T_{Mm}}(\sigma,L)$. 

Fix $t\in T_{mM}(\sigma,L)$, and let
$[\mu]\in\PML(S)$ maximize $R_t$ -- so that
$$d(\sigma,L) = d(\sigma, L(t)) = \half \log R_t(\mu).$$
Since $d(\sigma,L(s_\lambda))\ge d(\sigma,L)$, and using
lemma \ref{Ratio estimates distance}, we obtain
$$c_3R_{s_\lambda}(\lambda) \ge R_t(\mu)$$
for any $\lambda\in {\til A_{Mm}}(\sigma,L)$. But by choice of $\mu$, $R_t(\mu)\ge
R_t(\lambda)$. Finally, $R_t(\lambda)\ge r_t(\lambda)\ge
\half r_{s_\lambda}(\lambda)\exp 2|t-s_\lambda|$, and
$R_{s_\lambda}(\lambda) \le c_0r_{s_\lambda}(\lambda)$. We conclude
$$c_0c_3 \ge \half \exp 2|t-s_\lambda|.$$
This bounds $|t-s_\lambda|$ by some $c_5$, and the proof of theorem
\ref{Characterize projection} is complete. 
\end{pf} % characterize projection

\section{The contraction theorem}
\label{projecting}
Our main theorem follows almost directly from 
the results of the previous section.

\begin{theorem}{Contraction at a distance}{}
Given $\ep$ there are constants $b_1,b_2$ depending on
$\ep,\chi(S)$ such that for any 
$\ep$-precompact geodesic $L$, if $\sigma\in \TT(S)$ is such that
$d(\sigma,L)> b_1$ then, setting $r=d(\sigma,L)-b_1$,
$$\diam(\pi_L(\nbd_r(\sigma)))\le b_2.$$
In particular, for some $b_0= b_0(\ep,\chi(S))$ and all
$\sigma\in\TT(S)$ we have
$$\diam(\pi_L(\sigma))\le b_0.$$
\end{theorem}

\begin{pf}{}
Since $\pi_L(\sigma) = \{L(t): t\in T_{mM}(\sigma,L)\}$, and $t$
measures Teichm\"uller arclength along $L$, 
the bound on $\diam(\pi_L(\sigma))$ follows directly from 
theorem \ref{Characterize projection}. (Note also that it is a logical
consequence of the first diameter bound, with $b_0=\max(b_2,2b_1)$).

Let $\tau$ be such that $d(\sigma,\tau)\le r.$ Suppose $\lambda\in{\til A_{Mm}}
(\sigma,L)$ and $\mu\in{\til A_{Mm}}(\tau,L)$.  By the proof of theorem
\ref{Characterize projection}, it is sufficient to find a
value for $b_1$ that allows us to bound $|s_\lambda-s_\mu|$ (note that
$s_\lambda$ and $s_\mu$ are indpendent of $\sigma$ and $\tau$).

Suppose $|s_\lambda - s_\mu|>D$, where $D$ is the constant in lemma
\ref{Distance implies intersection}. 
Then corollary \ref{product bound} again gives
$$R_{\sigma,s_\lambda}(\lambda)R_{\sigma,s_\lambda}(\mu) \le {1\over c_1}.$$
By choice of $\lambda$, and lemma \ref{Ratio estimates distance},
$$R_{\sigma,s_\lambda}(\lambda) \ge c_3^{-1} \exp 
2d(\sigma,L),$$ 
and similarly with $\sigma$ and
$\lambda$ replaced by $\tau$ and $\mu$.
We note also that 
$$E_\sigma(\mu)\le e^{2r} E_\tau(\mu)$$
by choice of $\tau$ and by (\ref{K ratio}), and therefore
$$R_{\tau,s_\lambda}(\mu) \le e^{2r} R_{\sigma,s_\lambda}(\mu).$$
By definition of
$s_\mu$ and by lemma 
\ref{Extremal length estimate}, 
$$R_{\tau,s_\mu}(\mu)\le c_0 R_{\tau,s_\lambda}(\mu).$$
Putting all this together, we obtain
\begin{align*}
d(\sigma,L) + d(\tau,L) & \le  \half\log (c_3^2
R_{\sigma,s_\lambda}(\lambda)R_{\tau,s_\mu}(\mu) ) \\
& \le \half\log (c_3^2c_0e^{2r}
R_{\sigma,s_\lambda}(\lambda)R_{\sigma,s_\lambda}(\mu) ) \\
& \le r + C
\end{align*}
where $C = \half\log(c_3^2c_0/c_1).$
Now if we choose $b_1 > C/2$ and assume  $d(\sigma,L) > b_1$, then 
since $r=d(\sigma,L)-b_1$ we have $d(\tau,L) \le C - b_1 < b_1$. But, by
the choice of $\tau$ and the triangle inequality, 
$d(\tau,L)\ge b_1$. This contradiction implies that
$|s_\lambda - s_\mu| \le D$. 
\end{pf}



==> sharp.tex <==
\section{The case of non-precompact geodesics}
\label{sharpness}

In this section we consider the sharpness of theorem \ref{Contraction
at a distance}. Let $L$ be a geodesic which is not precompact. Then
$L$ has segments which enter, arbitrarily deeply, into the ``thin
parts'' $Thin(\alpha,\delta)$ defined in the previous section.

For small $\delta$, the geometry of $Thin(\alpha,\delta)$ is quite
far from negatively curved. In \cite{minsky:extremal} we showed that
it is approximated by a product space in the following sense.

Let $X_\alpha$ denote $\Hyp^2\times
\TT(S\setminus\alpha)$, endowed with the {\em sup metric} $d_X =
\max(d_{\Hyp^2},d_{\TT(S\setminus\alpha)})$ of the metrics on the
factors. There is a natural homeomorphism $\Pi:\TT(S)\to X_\alpha$,
defined using Fenchel-Nielsen coordinates, so that the coordinates in
the hyperbolic plane $\Hyp^2$ encode the length and twist parameters
associated to $\alpha$. In particular, the $y$ coordinate in $\Hyp^2$
(in the upper half-plane model) for $\Pi(\sigma)$ is
$1/\ell_\sigma(\alpha)$ where $\ell_\sigma$ is hyperbolic length, and
it follows easily that $\Pi(Thin(\alpha,\delta))$ is contained in
$\{y>\ell_1\}\times\TT(S\setminus\alpha)$ and contains
$\{y>\ell_2\}\times\TT(S\setminus\alpha)$, where $\ell_1,\ell_2$
are approximately inversely proportional to $\delta$.
The main theorem of \cite{minsky:extremal} says that

\begin{theorem}{product region}
{\rm (Theorem 6.1 of \cite{minsky:extremal})}
For sufficiently small $\delta$, the map $\Pi$ 
restricted to $Thin(\alpha,\delta)$ has bounded 
additive distortion; that is, 
$$
|d_{\TT(S)}(\sigma,\tau) - d_X(\Pi(\sigma),\Pi(\tau))| \le c
$$
for $\sigma,\tau\in Thin(\alpha,\delta)$, where $c$ depends only on
$\delta$ and the topological type of $S$. 
\end{theorem}

This product geometry suffices to give a converse to 
theorem \ref{Contraction at a distance}:

\begin{theorem}{contraction converse}
If a Teichm\"uller geodesic $L$ is not precompact, then there is no
choice of constants $b_1,b_2$ for which the contraction property of 
theorem \ref{Contraction at a distance} holds for $\pi_L$.
\end{theorem}

Remark: This theorem does not rule out the diameter bound for images
of single points which is stated in theorem \ref{Contraction at a
distance}. In fact it is not ruled out that $\pi_L(\sigma)$ is in all cases
a single point; resolving this question seems to require finer
techniques than we use here. 

\begin{pf}
Using the product structure we can show that large segments of $L$ can
be replaced by quasi-geodesics that stray arbitrarily far from $L$.
This will contradict theorem \ref{Stability of quasi-geodesics}.

Since $L$ is not precompact, for arbitrarily small $\delta>0$ and
large $T>0$ there exists a segment in $L$ of length $T$ contained in
$Thin(\alpha,\delta)$ for some $\alpha$. (We are using here the fact
that the Teichm\"uller metric on the moduli space is complete, or
equivalently that the distance from the boundary of
$Thin(\alpha,\delta)$ to $Thin(\alpha,\delta')$ goes to infinity as
$\delta/\delta'\to\infty$ -- in fact it is $\half\log(\delta/\delta')$.)

Let $\sigma_1,\sigma_2$ be the endpoints of such a segment, and let
$\Pi(\sigma_i) = q_i$ be their images in the product $X_\alpha$,
so that $|d(q_1,q_2) - T| < c$. 
Using the sup metric on $X_\alpha$ it is easy to construct two
$(2,0)$-quasi-geodesics $m,m'$ connecting $q_1$ to $q_2$, so that 
neither quasi-geodesic lies in a $(T-c)$-neighborhood of the other. 
(restricting to an $\R^2$ slice, construct an appropriate
quadrilateral whose diagonal is 
the line $[q_1,q_2]$, and let $m,m'$ be the two paths around the perimeter).
Furthermore $m,m'$ can be made to remain in $\Pi(Thin(\alpha,\delta'))$
for $\delta'$ slightly bigger than $\delta$. Then applying $\Pi^{-1}$, 
we obtain two $(2,c)$-quasi-geodesics connecting $\sigma_1$ to
$\sigma_2$, neither of which lies in a $(T-2c)$-neighborhood of the
other. It follows that at least one of the quasi-geodesics cannot be
in a bounded neighborhood of $L$, as $T$ is chosen arbitrarily large. 
This violates the stability of quasi-geodesics 
proved in Theorem \ref{Stability of quasi-geodesics}, and therefore
$\pi_L$ cannot have the contraction property.
\end{pf}

Remark: For a product space with the sup metric the stability of
quasi-geodesics is actually violated in a stronger way than used
above. See the last section of \cite{minsky:extremal} for a brief
discussion of this. 
